Stars: Tera-Scale Graph Building for Clustering and Graph Learning

A fundamental procedure in the analysis of massive datasets is the construction of similarity graphs. Such graphs play a key role for many downstream tasks, including clustering, classification, graph learning, and nearest neighbor search. For these tasks, it is critical to build graphs which are sparse yet still representative of the underlying data. The benefits of sparsity are twofold: firstly, constructing dense graphs is infeasible in practice for large datasets, and secondly, the runtime of downstream tasks is directly influenced by the sparsity of the similarity graph. In this work, we present $\textit{Stars}$: a highly scalable method for building extremely sparse graphs via two-hop spanners, which are graphs where similar points are connected by a path of length at most two. Stars can construct two-hop spanners with significantly fewer similarity comparisons, which are a major bottleneck for learning based models where comparisons are expensive to evaluate. Theoretically, we demonstrate that Stars builds a graph in nearly-linear time, where approximate nearest neighbors are contained within two-hop neighborhoods. In practice, we have deployed Stars for multiple data sets allowing for graph building at the $\textit{Tera-Scale}$, i.e., for graphs with tens of trillions of edges. We evaluate the performance of Stars for clustering and graph learning, and demonstrate 10~1000-fold improvements in pairwise similarity comparisons compared to different baselines, and 2~10-fold improvement in running time without quality loss.

==> scrap.tex <==

\begin{comment}
%Consider the following problem. Let $P$ be the point set. Given points $x,y$ with $d(x,y) < r$, and an approximation ratio $C > 1$. Let $F_x \subset P$ be the set of ``far'' points $F_x= \{z \in P \; | \; d(z,x) > Cr \}$. Let $\mathcal{H}$ be a family of LSH hash functions for the set $P$, and let $(h_1,h_2,\dots)$ be a sequence of independent draws from $\mathcal{H}$. For each point $z \in P \setminus {X}$, let $N_z$ be the largest value of $i$ such that $(h_1(z),\dots,h_i(z)) = (h_1(x),\dots,h_i(x))$. In other words, $N_z$ is the length of the prefix of sketches shared by $z$ and $x$. We want to show the following:
%\begin{itemize}
    \item With probability at least $\delta$, we have $N_y < \min_{z \in F_x} N_z$.
\end{itemize}

%By repeating at least $1/\delta$ times, we can be sure that we will find at least one point in $P \setminus F_x$ to which we can create an edge with $x$.


\subsection{Preliminaries on LSH }
We begin by introducing the standard definition of a locally sensitive hash family for a metric space \cite{indyk1998approximate}.

\begin{definition}[Locally sensitive hashing \cite{indyk1998approximate,har2012approximate}]\label{def:LSH}
Let $\cX$ be a metric space, let $U$ be a range space, and let $r \geq 0$ $c \geq 1$ and $0 \leq p_2 \leq p_1  \leq 1$ be reals.
A family $\cH = \{h : \cX \to U\}$ is called $(r,cr,p_1,p_2)$-sensitive if for any $q,p \in \cX$:

\begin{itemize}
    \item If $d(p,q) \leq r$, then $\prb{\cH}{h(q) = h(p)} \geq p_1$. 
    \item If $d(p,q) > cr$, then $\prb{\cH}{h(q) = h(p)} \leq p_2$. 
\end{itemize}
\end{definition}

Given a $(r,cr,p_1,p_2)$-sensitive family $\cH$, we can define $\cH^t$ to be the set of all functions $h^t: \cX \to U^t$ defined by $h^t(x) = (h_1(x),h_2(x),\dots,h_t(x))$, where  $h_1,\dots,h_k \in \cH$. In other words, a random function from $\cH^t$ is obtained by drawing $t$ independent hash functions from $\cH$ and concatenating the results. It is easy to see that the resulting hash family $\cH^t$ is $(r,cr,p_1^t,p_2^t)$-sensitive. 
We now demonstrate how a $(r,c)$-approximate threshold graph can be defined via a locally sensitive hash function. 
\end{comment}


\begin{comment}
\begin{definition}[Locally sensitive hashing \cite{indyk1998approximate,har2012approximate}]\label{def:LSH}
Let $P$ be a set of points endowed with either a distance or similarity measure $D:P^2 \to \R$, and let $U$ be a range space. 
A family $\cH = \{h : P \to U\}$ is called $(r_1,r_2,p_1,p_2)$-sensitive if for any $q,p \in P$:

\begin{itemize}
    \item If $p \in \cB(q,r_1)$, then $\prb{\cH}{h(q) = h(p)} \geq p_1$. 
    \item If $p \notin \cB(q,r_2)$, then $\prb{\cH}{h(q) = h(p)} \leq p_2$. 
\end{itemize}
\end{definition}
Note that, in order for a locally sensitive hash family to be useful, we must have $p_1 > p_2$ and $r_1 < r_2$ when $D$ is a distance measure, and we must have $p_1 > p_2$ and $r_1 < r_2$ when $D$ is a similarity measure. 
\end{comment}


We split the proof of Theorem \ref{thm:lshMain} into two cases, given that we want a $O(1/\eps)$ approximation in $O(n^{1+O(\eps)})$ time. In \textbf{Case 1}, we have $n^{2 \epsilon} < k$, and in this case we demonstrate that SortingLSH $+$ Two-hop spanner succeeds in finding $k$-approximate nearest neighbors in the two-hop subgraphs of each vertex. In \textbf{Case 2}, we have $n^{2 \epsilon} \geq k$, and in this case we demonstrate that simply SortingLSH alone provides the $k$-approximate nearest neighbor guarantee in the one-hop neighborhoods of each vertex. We summarize these in the following theorems. 

\begin{theorem}
Fix any $\eps  \in (0,1)$, such that $n^{2 \epsilon} \leq k$. 
For $x\in P$, let $\tau_k(x)$ denote the similarity of the $k$-nearest neighbor of $x$, and let $\mathcal{H}$ be the SimHash family. Let $G = (P,E)$ be the graph produced by the above process. For $\alpha \geq 0$, let $G_{\alpha}$ denote the subgraph $(P,E_{\alpha})$ of $G$ given by $E_{\alpha} = \{(x,y) \in E \; | \; \mathrm{sim}(x,y)\geq \alpha \}$. Then we have: 
\begin{enumerate}
    \item For any $x \in P$,  we have
    
    \[ \left| \mathcal{N}^2_{G_{ \eps^{-1}\tau_k(x) }}(x) \cap \{y \in P \; | \; \mathrm{sim}(x,y)\geq  \eps^{-1} \tau_k(x) \}  \right|  \geq k \] 
    \item $|E(G)| =O(n^{1+O(\eps)})$
\end{enumerate}

\end{theorem}
When proving this, if $X$ is the number of $k$-NN which collide at the right level with a point, we have $E[X] > n^{-c} k$, and since $X\leq k $ always, we have $Pr[X > n^{-c} k /100] > n^{-c} /100$,  and so we repeat $100 n^{-c} k$ times to conclude. 


\begin{theorem}
Fix any $\eps  \in (0,1)$, such that $n^{2 \epsilon} \geq  k$. Then the SortingLSH algorithm produces a graph $G$ such that
\begin{enumerate}
    \item For any $x \in P$,  we have
    
    \[ \left| \mathcal{N}_{G_{ \tau_k(x)/\eps }}(x) \}  \right|  \geq k \] 
    \item $|E(G)| =O(n^{1+O(\eps)})$
\end{enumerate}

\end{theorem}
\subsection{Analysis in Case $1$}




 %Specifically, given a approximation factor $c \geq 1$, and a metric $(P,d)$, one would like to find as many points $x \in P$ as possible which satisfy $\mu(p,x_i) \leq c \cdot \tau_k(p)$ (ideally, one would find at least $k$ of them). 
%For $c=1$, this is the exact $k$-NN problem, and for $c > 1$, the problem allows one to return any point which is distance at most $c$ times larger than the distance from $p$ to its $k$-th nearest neighbor. 
%In this setting, given an LSH family $\cH$ for $(P,d)$, one would like to find some $\rho = \rho(c,k,P,\cH)$, such that the set $\cA_p = \{x \in P \;| \; \mu(p,x) \leq c \cdot \tau_k(p) \}$ is a $(k,\rho)$-ANN. 

%For many similarity measures, it is known that there are hash families $\cH$ such that the set $\{x \in P \;| \; \mu(p,x) \leq c \cdot \tau_k(p) \}$ of $c$-approximate nearest neighbors is a $(k,\rho)$-ANN. for $\rho = O(1/c)$. This is true of the Hamming metric, Jaccard Distance, Euclidean space $(\R^d, \ell_2)$, and more generally $\ell_p$ metrics for constant $p \geq 1$ $(\R^d, \ell_p, )$. 

\begin{comment}
	

\begin{proposition}
Let $P \subset \R^d$ be equipped with the $\ell_0$ norm dissimilarity $\mu(x,y) = \|x-y\|_0$, and define the coordinate-sampling hash family $\mathcal{H} = \{h_1,\dots,h_d\}$ where $h_i(x) = x_i$.  Fix any $\eps \in (0,1)$. Then, for any $p \in P$, the set
\[  \cA_p= \{ x \in P \; | \; \mu(p,x) \leq \eps^{-1} \cdot \tau_k(p) \} \]
is a $(k, O(\eps),d \log d)$-ANN set with respect to $\cH$.
\end{proposition}
\begin{proof}
  Fix any $p \in P$, and set $\ell = \ell_p = 4 \eps \frac{d}{\tau_k(p) } \log n \leq d \log d$. Then note that, for any $x \in N_k(p)$, the probability that $h_1(p),\dots,h_\ell(p) =h_1(x),\dots,h_\ell(x)$ is at least $(1-\frac{\tau_k(p)}{d})^{\ell} = n^{-O(\eps)}$. On the other hand, for any $y \notin \cA_p$, the probability that $h_1(p),\dots,h_\ell(p) =h_1(y),\dots,h_\ell(y)$  is at most $(1-\eps \frac{\tau_k(p)}{\eps d})^{\ell} < (1/2)^{ 4 \log n} = 1/n^4$, where we used the inequality that $(1-x)^{n/x}  \leq \left(\frac{1}{2}\right)^n$ for any $x \in (0,1]$ and $n \geq 1$, which completes the proof. \end{proof}

\end{comment}
%\begin{proposition}
%Let $P \subset \{-\Delta,\dots,\Delta\}^d$ be equipped with the $\ell_1$ norm dissimilarity $\mu(x,y) = \|x-y\|_1$, and define the hash family $\mathcal{H}$ where $h \sim \cH$ is selected by  drawing $i \sim [d]$ and $r \sim \{-\Delta,\dots,\Delta\}$ uniformly at random, and setting $h(x) = \mathbf{1}(x_i \geq r)$.  Then for any $\eps \in (0,1)$, integer $M \geq 1$,  and $p \in P$, the set
%\[  \cA_p= \left\{ x \in P \; | \; \mu(p,x) \leq \max\left\{  \eps^{-1} \cdot \tau_k(p) , \frac{\Delta d}{M}\right\} %\right\} \]
%is a $(k, O(\eps),O(d \log d))$-ANN set with respect to $\cH$.
%\end{proposition}

